Spanish TrOCR: Leveraging Transfer Learning for Language Adaptation

This study explores the transfer learning capabilities of the TrOCR architecture to Spanish. TrOCR is a transformer-based Optical Character Recognition (OCR) model renowned for its state-of-the-art performance in English benchmarks. Inspired by Li et al. assertion regarding its adaptability to multilingual text recognition, we investigate two distinct approaches to adapt the model to a new language: integrating an English TrOCR encoder with a language specific decoder and train the model on this specific language, and fine-tuning the English base TrOCR model on a new language data. Due to the scarcity of publicly available datasets, we present a resource-efficient pipeline for creating OCR datasets in any language, along with a comprehensive benchmark of the different image generation methods employed with a focus on Visual Rich Documents (VRDs). Additionally, we offer a comparative analysis of the two approaches for the Spanish language, demonstrating that fine-tuning the English TrOCR on Spanish yields superior recognition than the language specific decoder for a fixed dataset size. We evaluate our model employing character and word error rate metrics on a public available printed dataset, comparing the performance against other open-source and cloud OCR spanish models. As far as we know, these resources represent the best open-source model for OCR in Spanish. The Spanish TrOCR models are publicly available on HuggingFace [20] and the code to generate the dataset is available on Github [25].

==> content/background.tex <==
\subsection{Models}

\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & \textbf{Total Parameters} & \textbf{Encoder} & \textbf{Decoder} \\
\hline
\textbf{TrOCR SMALL} & 62M & DeiT SMALL & MiniLM \\
\hline
\textbf{TrOCR BASE} & 334M & BEiT BASE & RoBERTa LARGE \\
\hline
\textbf{TrOCR LARGE} & 558M & BEiT LARGE & RoBERTa LARGE \\
\hline
\textbf{DeiT+MiniLM SMALL} & 48M & DeiT SMALL & MiniLM \\
\hline
\textbf{BeiT+RoBERTa BASE} & 239M & BeiT BASE & RoBERTa BASE \\
\hline
\end{tabular}
\caption{Small, base, and large versions of the TrOCR architecture alongside the two models resulting from the combination of an English encoder and a Spanish decoder.}
\label{table:trOCR_models}
\end{table}


\noindent This study delves into the TrOCR architecture, introduced by Li et al. \cite{li2022trocr} in 2021, marking a significant stride in OCR technology. The architecture features three variants: small, base, and large versions, primarily differentiated by the number of trainable parameters, as outlined in Table \ref{table:trOCR_models}. Notably, the small variant is approximately nine times lighter than the large model. This diversity enables us to strike a balance between resource efficiency and parameter richness, thus enhancing the model's capability to understand language nuances and image details. Within the TrOCR architecture, all variants leverage vision transformers in their encoders, each with its unique architectural components (Table \ref{table:trOCR_models}). The small version adopts the DeiT architecture \cite{DeiT}, while the base and large versions incorporate a BeiT \cite{BeiT} model. Additionally, there is variation among the decoders: the small version integrates MiniLM \cite{miniLM}, while the base and large versions use RoBERTa \cite{roberta}. These three models have been trained on a dataset comprising hundreds of millions of English samples and are publicly available on the HuggingFace platform. For instance, the URL of the small version can be found here: \url{huggingface.co/microsoft/trocr-small-stage1}.

The TrOCR architecture stands as our initial testing ground. The second architecture involves merging an English TrOCR encoder with a Spanish decoder. The crucial components facilitating this merge are the cross-attention layers, responsible for establishing the connection between the encoder and the decoder. In our approach, we opt to link the output of the encoder directly to the input of the cross-attention layers of the decoder. Initially, the weights of these layers are randomly initialized, and subsequent training is required to optimize their performance.

To ensure a fair comparison of these models, the encoder and decoder used must be similar in size and performance to those employed by the TrOCR models. To achieve this, the focus has to be directed towards a Spanish version of the MiniLM and the RoBERTa base model. This selection yields two models: a DeiT+MiniLM model, comparable to the small version of the TrOCR, and a BeiT+RoBERTa base model, akin to the base version of the TrOCR. As illustrated in Table \ref{table:trOCR_models}, these models not only share comparable architectures but also possess similar numbers of trainable parameters.

\subsection{Dataset}

To ensure the comprehensiveness of our study, acquiring an external Spanish dataset is essential for conducting accurate and relevant benchmark comparisons between our models. After thorough research within the open-source community, we identified the XFUND dataset \cite{xfund}, a significant contribution offering a multilingual benchmark for form understanding. Developed as part of the LayoutXLM project \cite{xu2021layoutxlm}, XFUND comprises human-labeled forms with key-value pairs in various languages. Our primary focus is on the Spanish segment of the XFUND dataset, which is dedicated solely to printed samples.
\\
A comparable dataset, known as the FUNSD dataset \cite{funsd}, has also been released specifically in the English language. However, as it closely resembles the XFUND dataset, we will not delve further into its exploration, as the sole distinction lies in the language of the samples.
\\
However, the XFUND dataset consists of only about 10,000 images, which is insufficient for effectively fine-tuning the English TrOCR models and training the English-encoder Spanish-decoder models. Motivated by the objective of establishing a comprehensive platform for OCR fine-tuning across various languages, including Latin and others, we decided to create our own dataset. As a result, we intend to use the XFUND dataset exclusively for benchmarking purposes.

\subsection{Evaluation metrics}

The models are evaluated using the Character Error Rate (CER) and Word Error Rate (WER) metrics. These metrics measure the minimum number of insertions, deletions, and substitutions required to transition from the model's predicted text to the ground truth. To mitigate bias related to text length, a normalization factor is applied, based on the length of the ground truth.
\\
\[
    \text{CER} = \frac{I + S + D}{N} = \frac{I + S + D}{S + D + C} \quad,
\] 
    
\noindent where:

\begin{itemize}
\item $S$ is the number of character substitutions.
\item $D$ is the number of character deletions.
\item $I$ is the number of character insertions.
\item $C$ is the number of correct characters.
\item $N$ is the number of characters in the ground truth.
\end{itemize}

\[
    \text{WER} = \frac{I + S + D}{N} = \frac{I + S + D}{S + D + C} \quad,
\] 
    
\noindent where:
    
\begin{itemize}
\item $S$ is the number of word substitutions.
\item $D$ is the number of word deletions.
\item $I$ is the number of word insertions.
\item $C$ is the number of correct words.
\item $N$ is the number of words in the ground truth.
\end{itemize}

\noindent It is essential to highlight that our evaluation methodology involves computing the mean CER and WER across samples in the test dataset. Alternatively, a common approach is to calculate the weighted average based on sample length. This helps to reduce length-related bias
and typically yields smaller metric values, but can be subject to misinterpretation as it does not reflect the mean value of the metric across the entire test dataset.

==> content/discussion.tex <==
\subsection{Text length effect of model specialization}

The uniform text length distribution in the training dataset for the Spanish versions of the TrOCR warrants discussion. To address this, we conducted an experiment involving training the small version of the English TrOCR using our dataset generation method. Specifically, we trained the model on three distinct datasets: one comprising single-word instances, another consisting of sentences with ten words each, and a third containing a balanced distribution of text lengths ranging from one to ten words. The results of this experiment are presented in Figure \ref{fig:method_length_training}.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/method_length_training.png}
    \caption{The graph illustrates the CER and WER metrics attained by the small version of the English TrOCR, trained on various datasets. The blue line represents training on images containing only one word, the orange line on images containing only ten words, and the green line on a dataset comprising various types of images. Each data point on the graph denotes the mean value over 100 samples corresponding to the respective text length (measured in terms of the number of characters).}
    \label{fig:method_length_training}
\end{figure}

\noindent The analysis revealed that models trained exclusively on images with one or ten words lost their ability to recognize the opposite type of images. Surprisingly, these specialized models failed to outperform the generalistic model on a diverse dataset, with consistently superior metrics achieved by the latter in terms of CER and WER. Consequently, specialized models consistently exhibited inferior metrics, suggesting a counterproductive outcome. This conclusion is believed to hold true for other models due to the consistent trend observed across the results and the potentially reduced generalization capability inherent in smaller-sized models.

\subsection{English better than Spanish}

\subsection{Carbon footprint}

Given the inherent uncertainties associated with such a process, we estimate the carbon footprint of the research to be approximately 150 kg of CO2eq.\\
The widely accepted standard dictates that we should limit our carbon emissions to a maximum of 2 tons of CO2 per person per year. In comparison, the carbon footprint generated by this research is substantial. The question arises as to whether it is beneficial for society to expend such a significant amount of carbon emissions on the training of an OCR. On one hand, this contributes to the automation of complex tasks, potentially yielding substantial improvements in social and environmental challenges. On the other hand, critics may argue that this perspective relies heavily on techno-solutionism, where there is a prevailing belief that technology can solve all problems. This section is not intended to provide the reader with a definitive answer but rather to prompt reflection on the relevance of such a research process within the current context.
